Joint Analysis of Single-Cell Data across Cohorts with Missing Modalities

Joint analysis of multi-omic single-cell data across cohorts has significantly enhanced the comprehensive analysis of cellular processes. However, most of the existing approaches for this purpose require access to samples with complete modality availability, which is impractical in many real-world scenarios. In this paper, we propose (Single-Cell Cross-Cohort Cross-Category) integration, a novel framework that learns unified cell representations under domain shift without requiring full-modality reference samples. Our generative approach learns rich cross-modal and cross-domain relationships that enable imputation of these missing modalities. Through experiments on real-world multi-omic datasets, we demonstrate that offers a robust solution to single-cell tasks such as cell type clustering, cell type classification, and feature imputation.

==> algs/full_alg.tex <==
\begin{algorithm}
\caption{Topology-guided alignment of multi-domain \& multi-omic single cell features}\label{alg:align}
 \textbf{Input:} Single-cell observations $\{ \{ \mathbf{X}^{(d,m)} \in \mathbb{R}^{N^{(d,m)} \times V^{(d,m)}} \}_{m=1}^M \}_{d=1}^D$ \\
 \textbf{Input:} Graph message passing steps $\mathbf{k}$ \\
 \textbf{Output:} Domain-invariant features $\mathbf{Z} \in \mathbb{R}^{N \times H}$ \\
 \textbf{Output:} Denoised features $\{ \{ \mathbf{X'}^{m}_d \in \mathbb{R}^{N^{(d,m)} \times V^{(d,m)}} \}_{m=1}^M \}_{d=1}^D$ \\
\SetKwFunction{algo}{align\_all}\SetKwFunction{proco}{align\_omics}\SetKwFunction{procd}{align\_domains}
\SetKwProg{myalg}{Algorithm}{}{}
\myalg{\algo{}}{
  \nl \For{$d = 1$ \KwTo $D$}{
    \nl $\mathbf{Z}_d, \mathbf{X}'_{d} \gets$ \proco{$\mathbf{X}^{(d)}, \mathbf{k}$}\;
  }
  \nl $\mathbf{Z}, \mathbf{X'}, \mathbf{y}_{target} \gets$ \procd{$\mathbf{X}, \mathbf{y}_{source}, \{\mathbf{Z}^{(d)}\}_{d=1}^D$}\;
  \nl \KwRet $\mathbf{Z},\mathbf{X'}, \mathbf{y}_{target}$ \;}{}
\end{algorithm}

==> algs/modality_int.tex <==
\begin{algorithm}
\caption{Topology-guided alignment of multi-domain \& multi-omic single cell features}\label{alg:omic}
\textbf{Input:} Single-cell observations $\{ \mathbf{X}^{(d,m)} \in \mathbb{R}^{N^{(d,m)} \times V^{(d,m)}} \}_{m=1}^M$ \\
\textbf{Input:} Graph message passing steps $\mathbf{k}$ \\
\textbf{Output:} Modality-invariant features $\{ \mathbf{Z}^{(d)} \in \mathbb{R}^{N^{(d,m)} \times L} \}_{d=1}^D$ \\
\textbf{Output:} Intra-modality cell-cell relations $\{\mathcal{N}_{omic}^{(d)} \in \mathbb{R}^{N \times \mathbf{k}} \}_{d=1}^D$ \\
\SetKwFunction{proco}{align\_omics}

\SetKwProg{modality}{Procedure}{}{}
  \modality{\proco{}}{
   \nl \For{$m = 1$ \KwTo $M$}{
   \nl     $\mathbf{G}(\mathbf{X}^{(d,m)}) \gets \text{KNN} \left( \mathbf{X}^{(d,m)} \right)$ \;
    }
   \nl \For{$i = 1$ \KwTo $N$}{
        \nl $\mathcal{N}_{omic}(i) \gets \bigcup_{m=1}^M \text{NEIGHBORS} \left(i, \mathbf{G}(\mathbf{X}^{(d,m)}), \mathbf{k} \right)$ \;   
    }
    \nl \While{$\text{ENC}_{\theta}, \text{DEC}_{\omega}, \{\lambda\}_{m=1}^M$ not converged}{
        \nl $\mathbf{Z}^{(d)} \gets \text{ENC}_\theta^{(d,m)} \left( \text{AGG} \left( \mathbf{X}^{(d,1)}, \cdots, \mathbf{X}^{(d,M)}  \right), \mathcal{N}_{omic}(i)  \right)$\;
        \nl \For{$m = 1$ \KwTo $M$}{
            \nl $\hat{\mathbf{X}}^{(d,m)} \gets \text{DEC}^{(d,m)}_{\omega} \left( \mathbf{Z}^{(d)} \right) + \lambda^{(m)}$\;
        }
        \nl $l \gets \max_{1 \leq m \leq M} || \mathbf{X}^{(d,m)}-\hat{\mathbf{X}}^{(d,m)} ||^2$ \;
        \nl \For{$i = 1$ \KwTo $N$}{
            \nl$l \gets l + \text{CONTR} \left(\mathbf{Z}_i^{(d)}, \left[ \mathcal{N}_{omic}(i), \{ j \notin \mathcal{N}_{omic}(j)\}_{j=1}^N \right] \right)$\;
        }
        \nl $\theta \gets \theta -  \nabla l$ \;
        \nl $\omega \gets \omega -  \nabla l$ \;

    }
    \nl \KwRet $\mathbf{Z}^{(d)}$, $\mathcal{N}_{omic}$ \;
}
\end{algorithm}


==> discussion.tex <==
\section{Discussion}

==> related_work.tex <==
% \subsection{Motivation}
% We aim to learn a joint modality-invariant embedding of multi-omic observations, while leveraging a cell-cell similarity graph representing intra-omic relationships.

\subsection{Multi-modal integration under missing modality settings}

\marianne{
Recent methods in multi-modal integration under missing modality settings perform imputation as a pre-processing step.
SMIL \cite{ma2021smil} addresses bias from modality scarcity by performing missing modality imputation before learning joint embeddings. MultiModN \cite{swamy2023multimodn} proposes a multimodal fusion architecture that maintains robustness to the bias of missing modalities by sequentially encoding each modality, skipping over missing modalities. However, these methods  In contrast, our approach learns structured contextual relationships between modalities and samples through the generative model. This ensures consistency the learned multimodal relationship between samples with variable modality availability.

Recent methods in multi-modal integration for single-cell data under missing modality settings use full-modality reference samples to learn integrated features for samples with missing modalities. Multigrate \cite{Lotfollahi2022multigrate} uses a product-of-experts encoder to integrate available modalities and a conditional autoencoder to incorporate batch information. During testing, they fine-tune their model by incorporating new test batch labels. However, the conditional autoencoder can suffer from batch label bias based on the number of cells in each batch, and has limited interpretability due to the neural network decoder. Ding et. al use knowledge transfer to produce embeddings for a missing modality in a target domain by using an available common modality to learn a low-rank factor that guides the transfer \cite{ding2015missinglowrank}. Konwer et. al propose an adversarial architecture that learns modality-agnostic embeddings by using a discriminator to predict the absence/presence of modalities \cite{konwer2023mamlbrain}. However, their approach requires their discriminator to be trained over $2^M-1$ possible missing modality combinations for $M$ modalities. 

Cobolt \cite{gong2021cobolt} is a hierarchical Bayesian generative model that handles missing modalities by estimating posteriors for each unique modality availability setting.
scMoMAT \cite{zhang2023scmomat}  pre-computes missing features before performing cross-modal integration.
moETM \cite{zhou2023moetm} deals with missing modalities by training a model to reconstruct one modality from another. However, these methods require samples with full modality availability at training.

\marianne{(TODO: organize)}
Previous works have attempted to align modality/domain-specific features from different graphs. MSNE \cite{xu2021msne}, purposed for cross-domain transfer for bulk sequencing data, handles partial observations (missing samples from one omic) using a cross-domain random walk. ...

Optimal transport methods for single-cell integration have been extended with to compare metric spaces without full correspondences.
CMOT \cite{cmot} Pamona \cite{cao2022pamona} employs partial Gromov-Wasserstein optimal transport to find \textit{partial} cell-cell correspondences. SCOTv2 \cite{demetci2022scotv2} similarly applies unbalanced Gromov-Wasserstein optimal transport to align datasets without paired cell correspondences. UnionCom \cite{} uses a probabilistic matching matrix in applying an unsupervised alignment algorithm. However, .. (computational cost)

[In contrast, our method performs information sharing across batches using a fixed number of 'topics' via topic modeling, and interpretably models relationships between samples across modalities and domains using domain-specific topic embeddings and modality-specific feature embeddings during decoding.]}

\subsection{Multi-omic integration under domain shift}
Seuratv3 \cite{stuart2019seuratv3} identifies 'anchoring' cells between different domains with similar nearest neighbor to guide the alignment. scMMGAN \cite{amodio2022scmmgan} performs alignment of low-frequency feature signals (i.e. global features), while preserving the intra-domain cell-cell relationships as much as possible. Importantly, they note that alignment should flexibly match probability distributions between domains and preserve intra-domain relationships without strictly guiding the alignment on one or the other.

MARS \cite{brbic2020mars} aims to learn domain-invariant single-cell representations by transferring supervised cell type clustering in one domain to unsupervised cell type clustering in another domain without annotations. In particular, they use a single autoencoder to learn lower-dimensional representations for both supervised and unsupervised cell clustering. In inference, they classify unannotated cells by comparing their clusters with those of annotated cells. By comparing cell clusters in the embedding space, MARS can identify correspondences between annotated and unannotated cell types, while enabling novel cell type discovery for cell types not represented in annotated datasets.

scHPL \cite{} combines single-cell data from multiple annotated experiments via a hierarchical classifier that progressively learns hierarchical cell-cell relationships.

Portal \cite{zhao2022portal} employs a domain-adversarial neural network to, composed of a domain-translation network and a domain discriminator. The domain-translation network uses an encoder to predicts a denoised cell embedding in one domain, which is passed into a generator that generates cell embeddings in another domain. This framework learns the relationship between the data generating processes of separate domains. The domain discriminator distinguishes cell embeddings by their domain to encourage mixing of the generated distributions. Furthermore, they consider the task of integrating single-cell data across organs, tissue types, and species, even if they do not share the same cell types.

Conos \cite{barkas2019conos} learns cell-cell correspondences across heterogeneous domain shift (sample classes, disease groups, and tissues) by constructing and refining an atlas-level graph of intra-domain and inter-domain cell-cell relationships. They utilize the graphs structure to identify hierarchical cell populations, such as finer-grained cell subpopulations.

scPoli \cite{} uses a conditional variational autoencoder to encode domain-specific factors into a condition variable, in order to transfer domain-invariant features to new domains.


JIND...

STitch3D ...

